Finite Element Exterior Calculus for Evolution Problems

Arnold, Falk, and Winther [Bull. Amer. Math. Soc. 47 (2010), 281--354] showed that mixed variational problems, and their numerical approximation by mixed methods, could be most completely understood using the ideas and tools of Hilbert complexes. This led to the development of the Finite Element Exterior Calculus (FEEC) for a large class of linear elliptic problems. More recently, Holst and Stern [Found. Comp. Math. 12:3 (2012), 263--293 and 363--387] extended the FEEC framework to semi-linear problems, and to problems containing variational crimes, allowing for the analysis and numerical approximation of linear and nonlinear geometric elliptic partial differential equations on Riemannian manifolds of arbitrary spatial dimension, generalizing surface finite element approximation theory. In this article, we develop another distinct extension to the FEEC, namely to parabolic and hyperbolic evolution systems, allowing for the treatment of geometric and other evolution problems. Our approach is to combine the recent work on the FEEC for elliptic problems with a classical approach to solving evolution problems via semi-discrete finite element methods, by viewing solutions to the evolution problem as lying in time-parameterized Hilbert spaces (or Bochner spaces). Building on classical approaches by Thomee for parabolic problems and Geveci for hyperbolic problems, we establish a priori error estimates for Galerkin FEM approximation in the natural parametrized Hilbert space norms. In particular, we recover the results of Thomee and Geveci for two-dimensional domains and lowest-order mixed methods as special cases, effectively extending their results to arbitrary spatial dimension and to an entire family of mixed methods. We also show how the Holst and Stern framework allows for extensions of these results to certain semi-linear evolution problems.

==> symbols.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BEGIN: TeX/LaTeX/PDFLaTeX <Symbols> for Holst Group Papers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Notes.
%
%   These macros put together originally by G. Nagy.
%   Added to by M. Holst, G. Tsogtgerel, E. Lunasin, others.
%
% Conventions.
% -----------
% Field sets   : Mathbb upper case.
%                A,B,C,F,K,N,Z 
% Vector spaces: Sans Serif upper case.
%                H,M,N,V,W,X,Y,Z 
% Banach space : The pair X,\|~\|_X
% Hilbert space: The pair \bigl(H,(~,~)_H\bigr)
% Manifolds    : Caligraphic upper case.
%                and Greek upper case.
%                M,N,S,Sigma
% Riemannian manifold: (\cM,g)
% Operators    : Roman upper case.
%                A,B,C,J,I,L,O,P,Q,R,S,T
% Unbounded operators: (A,D_a)
% Bilinear forms: a(,), b(,), c(,)
% Linear functionals: \ell
% Vectors in R^n: boldface lower case.
%                 u,v,w,x,y,z
% Vectors in general: lower case roman.
%                     u,v,w,x,y,z   
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mathematical environment.
%\newcommand{\Sec}{Sec.~}
\newcommand{\Sec}{\S}
%\newcommand{\Sec}{Sec.~}
\newcommand{\Label}[1]{\label{#1}\mbox{\fbox{\bf #1}\quad}}
\renewcommand{\Label}[1]{\label{#1}}
% \newcommand{\eqref}[1]{(\ref{#1})}
\newcommand*{\ang}[1]{\left\langle #1 \right\rangle}
\renewcommand{\labelitemii}{$\bullet$}  % labels in itemize. 
%\renewcommand{\theenumi}{{\it(\roman{enumi})}}  % (i) labels in enumerate. 
%\renewcommand{\theenumi}{(\arabic{enumi})}
%\numberwithin{equation}{section}  %amsmath command: counter tied to section.
%
%\def\bold#1{{\bf #1}}
%\def\text#1{{\rm #1}}
%\def\calg#1{{\cal #1}}
%\def\bbbb#1{{\mathbb #1}}
\newcommand{\mbf}{\mathbf}
\newcommand{\mcal}{\mathcal}
\newcommand{\mbb}{\mathbb}
\def\mathbi#1{\textbf{\em #1}}
%
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
%
%\newtheorem{thrm}{Theorem}
%\newtheorem*{assumptionM}{Assumption M}
%\newtheorem*{assumptionH}{Assumption H}
%\newtheorem{xca}{Exercise}
%\numberwithin{equation}{section}
%

\newcommand{\p}{\alpha}
\newcommand{\pphi}{\dot{\phi}}
\newcommand{\PP}{\dot{P}}
\newcommand{\PPP}{\ddot{P}}
\newcommand{\Q}{\lambda}
\newcommand{\QQ}{\mu}
\newcommand{\QQQ}{\nu}
\newcommand{\CQ}{\Lambda}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mathematical symbol definitions.
\newcommand{\tbar}{|\hspace*{-0.15em}|\hspace*{-0.15em}|}
\newcommand{\normf}{\|f\|}
\newcommand{\del}{\rm del} 
\newcommand{\normx}{\|\mbf x\|^2}
%
\newcommand{\IB}{I\!\!B} 
\newcommand{\ID}{I\!\!D}          
\newcommand{\IE}{I\!\!E}         % Energy functional.
\newcommand{\IF}{I\!\!F}         % Fermi transport symbol.
\newcommand{\IH}{I\!\!H}          
\newcommand{\IK}{I\!\!K}          
\newcommand{\IL}{I\!\!L}
\newcommand{\IN}{I\!\!N}
\newcommand{\IP}{I\!\!P}          
\newcommand{\IR}{I\!\!R}         % Alternative real numbers symbol.
%
\newcommand{\sIB}{\sfI\!\sfB} 
\newcommand{\sID}{\sfI\!\sfD}          
\newcommand{\sIE}{\sfI\!\sfE}
\newcommand{\sIF}{\sfI\!\sfF}
\newcommand{\sIH}{\sfI\!\sfH}
\newcommand{\sIK}{\sfI\!\sfK}          
\newcommand{\sIL}{\sfI\!\sfL}
\newcommand{\sIP}{\sfI\!\sfP}          
\newcommand{\sIR}{\sfI\!\sfR}

%%%%%%%%%%%%%%%%%%%%%%%%%
% Linear Algebra
\newcommand{\codim}{\mbox{\rm codim\,}}
\newcommand{\Span}{\mbox{{\rm Span}}}
\newcommand{\Col}{\mbox{{\rm Col}}}
\newcommand{\Do}{{\cal D}}
\newcommand{\Ra}{{\cal R}}
\newcommand{\Nu}{{\cal N}}
\newcommand{\rank}{\mbox{{\rm rank}}}
\newcommand{\nullity}{\mbox{{\rm null}}}
\newcommand{\dist}{\mbox{{\rm dist}}}
\newcommand{\Vect}{\overrightarrow}

%%%%%%%%%%%%%%%%%%%%%%%%%
% Finite Elements
\newcommand{\vol}{\mbox{\rm vol\,}}
\newcommand{\gen}{\mbox{\rm gen\,}}
\newcommand{\diam}{\mbox{\rm diam\,}}
\newcommand{\val}{\mbox{\rm val\,}}

%%%%%%%%%%%%%%%%%%%%%%%%%
% Banach & Hilbert spaces
\newcommand{\ind}{\mbox{\rm ind\,}}           % Index of an operator
\newcommand{\bperp}{\bot\mspace{-8.5mu}\flat} % Banach perpendicular
\newcommand{\dual}{*}              % Dual vector spaces.
\newcommand{\Badj}{*}              % Banach Adjoint of an operator.
\newcommand{\Hadj}{\dagger}        % Hilbert adjoint of an operator.
\newcommand{\id}{\delta}           % Identity operator.
\newcommand{\Leven}{L_{\mbox{\tiny{\rm even}}}}
\newcommand{\Heven}{H_{\mbox{\tiny {\rm even}}}}
\newcommand{\closedw}{closed${}_{w}\,$}
\newcommand{\lscw}{lsc${}_{w}\,$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Manifolds and differential geometry
\newcommand{\Ri}{{}^{\mbox{\tiny \rm 3}}\!R} %3-Ricci.
\newcommand{\hRi}{{}^{\mbox{\tiny \rm 3}}\!\hat{R}} %3-hatted Ricci.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Other Mathematical commands
\newcommand{\Proof}{\noindent{\bf Proof.~}}
\newcommand{\wqed}{\hfill $\fbox{\hspace{0.3mm}}$ \vspace{.3cm}} 
\newcommand{\eqed}{\hfill $\fbox{\hspace{0.3mm}}$ \vspace{.3cm}} 
\newcommand{\Outline}{\noindent{\bf Outline of the Proof.~}}
\newcommand{\Remark}{\noindent{\bf Remark.~}}
\newcommand{\Solution}{\noindent{\bf Solution.~}}
%
\newcommand{\LRI}{\quad\Leftrightarrow\quad}
\newcommand{\LI}{\quad\Leftarrow\quad}
\newcommand{\RI}{\quad\Rightarrow\quad}
\newcommand{\wto}{\rightharpoonup} % Weak convergence.
\newcommand{\di}{\displaystyle}
\newcommand{\conv}{\rightarrow}
\newcommand{\weak}{\rightharpoonup}
\newcommand{\weakstart}{\rightharpoonup^{*}}
%
\newcommand{\leqs}{\leqslant}      % Nice >= 
\newcommand{\nleqs}{\nleqslant}     
\newcommand{\geqs}{\geqslant}      % Nice =<
\newcommand{\ngeqs}{\ngeqslant}      
%
\newcommand{\g}{\mbox{\textsf{g}}}    % Lie algebra.
\newcommand{\su}{\mbox{\textsf{su}}}  % Lie algebra.
\renewcommand{\div}{{\operatorname{div}}}
\newcommand{\sdiv}{\mbox{{\footnotesize div}}}   % subindex div.
\newcommand{\scurl}{\mbox{{\footnotesize curl}}} % subindex curl.
%\newcommand{\Tr}{{\sf tr}}
\newcommand{\Tr}{{\gamma}}
\newcommand{\ot}{\leftarrow}
\newcommand{\eps}{\varepsilon}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Tiny Fonts
\newcommand{\tif}{\mbox{{\tiny $f$}}}
%
\newcommand{\tibif}{\mbox{{\tiny $\bif$}}}
%
\newcommand{\tiA}{\mbox{{\tiny $A$}}}
\newcommand{\tiB}{\mbox{{\tiny $B$}}}
\newcommand{\tiC}{\mbox{{\tiny $C$}}}
\newcommand{\tiD}{\mbox{{\tiny $D$}}}
\newcommand{\tiE}{\mbox{{\tiny $E$}}}
\newcommand{\tiF}{\mbox{{\tiny $F$}}}
\newcommand{\tiG}{\mbox{{\tiny $G$}}}
\newcommand{\tiH}{\mbox{{\tiny $H$}}}
\newcommand{\tiI}{\mbox{{\tiny $I$}}}
\newcommand{\tiJ}{\mbox{{\tiny $J$}}}
\newcommand{\tiK}{\mbox{{\tiny $K$}}}
\newcommand{\tiL}{\mbox{{\tiny $L$}}}
\newcommand{\tiM}{\mbox{{\tiny $M$}}}
\newcommand{\tiN}{\mbox{{\tiny $N$}}}
\newcommand{\tiO}{\mbox{{\tiny $O$}}}
\newcommand{\tiP}{\mbox{{\tiny $P$}}}
\newcommand{\tiQ}{\mbox{{\tiny $Q$}}}
\newcommand{\tiR}{\mbox{{\tiny $R$}}}
\newcommand{\tiS}{\mbox{{\tiny $S$}}}
\newcommand{\tiT}{\mbox{{\tiny $T$}}}
\newcommand{\tiU}{\mbox{{\tiny $U$}}}
\newcommand{\tiV}{\mbox{{\tiny $V$}}}
\newcommand{\tiW}{\mbox{{\tiny $W$}}}
\newcommand{\tiX}{\mbox{{\tiny $X$}}}
\newcommand{\tiY}{\mbox{{\tiny $Y$}}}
\newcommand{\tiZ}{\mbox{{\tiny $Z$}}}
%
\newcommand{\tcX}{\mbox{{\tiny $\cX$}}}
\newcommand{\tcY}{\mbox{{\tiny $\cY$}}}
%
\newcommand{\tiID}{\mbox{{\tiny $\ID$}}}
\newcommand{\tiIE}{\mbox{{\tiny $\IE$}}}
\newcommand{\tiIF}{\mbox{{\tiny $\IF$}}}
\newcommand{\tiIK}{\mbox{{\tiny $\IK$}}}
\newcommand{\tiIL}{\mbox{{\tiny $\IL$}}}
\newcommand{\tiIN}{\mbox{{\tiny $\IN$}}}
%
\newcommand{\tsfH}{\mbox{{\tiny $\sfH$}}}
\newcommand{\tsfX}{\mbox{{\tiny $\sfX$}}}
\newcommand{\tsfY}{\mbox{{\tiny $\sfY$}}}
\newcommand{\tsfZ}{\mbox{{\tiny $\sfZ$}}}
%
\newcommand{\titH}{\mbox{{\tiny $\ttH$}}}
\newcommand{\titN}{\mbox{{\tiny $\ttN$}}}
\newcommand{\titX}{\mbox{{\tiny $\ttX$}}}
\newcommand{\titY}{\mbox{{\tiny $\ttY$}}}
\newcommand{\titZ}{\mbox{{\tiny $\ttZ$}}}
%
\newcommand{\tLt}{\mbox{{\tiny $L^2$}}}
\newcommand{\tHt}{\mbox{{\tiny $H^2$}}}
\newcommand{\tiwedge}{\mbox{{\tiny $\wedge$}}}
\newcommand{\tivee}{\mbox{{\tiny $\vee$}}}
\newcommand{\tiup}{\mbox{{\tiny $\vartriangle$}}}
\newcommand{\tidown}{\mbox{{\tiny $\triangledown$}}}
\newcommand{\tLtom}{\mbox{{\tiny $L^2(\Omega)$}}}
\newcommand{\tHtom}{\mbox{{\tiny $H^2(\Omega)$}}}
%
\newcommand{\tiDelta}{\mbox{{\tiny $\Delta$}}}
\newcommand{\DeltaT}{\Delta T}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Various Nabla operators.
\newcommand{\bnabla}{{\boldsymbol \nabla}}
\newcommand{\onabla}{\overline{\nabla}}
\newcommand{\bonabla}{\overline{\bnabla}}
\newcommand{\tnabla}{\tilde{\nabla}}
%
\newcommand{\tW}{W}                % Trace of tensor W.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mathbb fonts: Set of numbers.
\newcommand{\A}{{\mathbb A}} 
\newcommand{\B}{{\mathbb B}}
%\newcommand{\C}{{\mathbb C}}
\newcommand{\D}{{\mathbb D}}
\newcommand{\E}{{\mathbb E}}       % Euclidean manifold.
\newcommand{\K}{{\mathbb K}}
\newcommand{\HH}{{\mathbb H}}
\newcommand{\N}{{\mathbb N}}       % Natural numbers.
\newcommand{\OO}{{\mathbb O}}       % Natural numbers.
%\newcommand{\PP}{{\mathbb P}}       % Natural numbers.
\newcommand{\R}{{\mathbb R}}       % Real numbers.
\newcommand{\Ss}{{S}}              % Real numbers.
\newcommand{\W}{{\mathbb W}}
\newcommand{\X}{{\mathbb X}}
\newcommand{\Y}{{\mathbb Y}}
\newcommand{\Z}{{\mathbb Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Caligraphic font: Manifolds, operators.
\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cD}{{\mathcal D}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cI}{{\mathcal I}}
\newcommand{\cJ}{{\mathcal J}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\cL}{{\mathcal L}}
\newcommand{\cM}{{\mathcal M}}
\newcommand{\cN}{{\mathcal N}}
\newcommand{\cO}{{\mathcal O}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cU}{{\mathcal U}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cW}{{\mathcal W}}
\newcommand{\cX}{{\mathcal X}}
\newcommand{\cY}{{\mathcal Y}}
\newcommand{\cZ}{{\mathcal Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Sans Serif font: For vector spaces
\newcommand{\sfA}{{\mathsf A}}
\newcommand{\sfB}{{\mathsf B}}
\newcommand{\sfC}{{\mathsf C}}
\newcommand{\sfD}{{\mathsf D}}
\newcommand{\sfE}{{\mathsf E}}
\newcommand{\sfF}{{\mathsf F}}
\newcommand{\sfG}{{\mathsf G}}
\newcommand{\sfH}{{\mathsf H}}
\newcommand{\sfI}{{\mathsf I}}
\newcommand{\sfJ}{{\mathsf J}}
\newcommand{\sfK}{{\mathsf K}}
\newcommand{\sfL}{{\mathsf L}}
\newcommand{\sfM}{{\mathsf M}}
\newcommand{\sfN}{{\mathsf N}}
\newcommand{\sfO}{{\mathsf O}}
\newcommand{\sfP}{{\mathsf P}}
\newcommand{\sfQ}{{\mathsf Q}}
\newcommand{\sfR}{{\mathsf R}}
\newcommand{\sfS}{{\mathsf S}}
\newcommand{\sfT}{{\mathsf T}}
\newcommand{\sfU}{{\mathsf U}}
\newcommand{\sfV}{{\mathsf V}}
\newcommand{\SU}{\mbox{\textsf{SU}}}  % Lie group.
\newcommand{\sfW}{{\mathsf W}}
\newcommand{\sfX}{{\mathsf X}}
\newcommand{\sfY}{{\mathsf Y}}
\newcommand{\sfZ}{{\mathsf Z}}
%
\newcommand{\sfa}{{\mathsf a}}
\newcommand{\sfb}{{\mathsf b}}
\newcommand{\sfc}{{\mathsf c}}
\newcommand{\sfd}{{\mathsf d}}
\newcommand{\sfe}{{\mathsf e}}
\newcommand{\sff}{{\mathsf f}}
\newcommand{\sfg}{{\mathsf g}}
\newcommand{\sfh}{{\mathsf h}}
\newcommand{\sfi}{{\mathsf i}}
\newcommand{\sfj}{{\mathsf j}}
\newcommand{\sfk}{{\mathsf k}}
\newcommand{\sfl}{{\mathsf l}}
\newcommand{\sfm}{{\mathsf m}}
\newcommand{\sfn}{{\mathsf n}}
\newcommand{\sfo}{{\mathsf o}}
\newcommand{\sfp}{{\mathsf p}}
\newcommand{\sfq}{{\mathsf q}}
\newcommand{\sfr}{{\mathsf r}}
\newcommand{\sfs}{{\mathsf s}}
\newcommand{\sft}{{\mathsf t}}
\newcommand{\sfu}{{\mathsf u}}
\newcommand{\sfv}{{\mathsf v}}
\newcommand{\sfw}{{\mathsf w}}
\newcommand{\sfx}{{\mathsf x}}
\newcommand{\sfy}{{\mathsf y}}
\newcommand{\sfz}{{\mathsf z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Typewriter font: For vector spaces
\newcommand{\ttA}{{\tt A}}
\newcommand{\ttB}{{\tt B}}
\newcommand{\ttC}{{\tt C}}
\newcommand{\ttD}{{\tt D}}
\newcommand{\ttE}{{\tt E}}
\newcommand{\ttF}{{\tt F}}
\newcommand{\ttG}{{\tt G}}
\newcommand{\ttH}{{\tt H}}
\newcommand{\ttI}{{\tt I}}
\newcommand{\ttJ}{{\tt J}}
\newcommand{\ttK}{{\tt K}}
\newcommand{\ttL}{{\tt L}}
\newcommand{\ttM}{{\tt M}}
\newcommand{\ttN}{{\tt N}}
\newcommand{\ttO}{{\tt O}}
\newcommand{\ttP}{{\tt P}}
\newcommand{\ttQ}{{\tt Q}}
\newcommand{\ttR}{{\tt R}}
\newcommand{\ttS}{{\tt S}}
\newcommand{\ttT}{{\tt T}}
\newcommand{\ttU}{{\tt U}}
\newcommand{\ttV}{{\tt V}}
\newcommand{\ttW}{{\tt W}}
\newcommand{\ttX}{{\tt X}}
\newcommand{\ttY}{{\tt Y}}
\newcommand{\ttZ}{{\tt Z}}
%
\newcommand{\tta}{{\tt a}}
\newcommand{\ttb}{{\tt b}}
\newcommand{\ttc}{{\tt c}}
\newcommand{\ttd}{{\tt d}}
\newcommand{\tte}{{\tt e}}
\newcommand{\ttf}{{\tt f}}
\newcommand{\ttg}{{\tt g}}
\newcommand{\tth}{{\tt h}}
\newcommand{\tti}{{\tt i}}
\newcommand{\ttj}{{\tt j}}
\newcommand{\ttk}{{\tt k}}
\newcommand{\ttl}{{\tt l}}
\newcommand{\ttm}{{\tt m}}
\newcommand{\ttn}{{\tt n}}
\newcommand{\tto}{{\tt o}}
\newcommand{\ttp}{{\tt p}}
\newcommand{\ttq}{{\tt q}}
\newcommand{\ttr}{{\tt r}}
\newcommand{\tts}{{\tt s}}
\newcommand{\ttt}{{\tt t}}
\newcommand{\ttu}{{\tt u}}
\newcommand{\ttv}{{\tt v}}
\newcommand{\ttw}{{\tt w}}
\newcommand{\ttx}{{\tt x}}
\newcommand{\tty}{{\tt y}}
\newcommand{\ttz}{{\tt z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Boldface Font
\newcommand{\bA}{{\bf A}}
\newcommand{\bB}{{\bf B}}
\newcommand{\bC}{{\bf C}}
\newcommand{\bD}{{\bf D}}
\newcommand{\bE}{{\bf E}}
\newcommand{\bF}{{\bf F}}
\newcommand{\bV}{{\bf V}}
\newcommand{\bW}{{\bf W}}
\newcommand{\bX}{{\bf X}}
%
\newcommand{\ba}{{\bf a}}
\newcommand{\bb}{{\bf b}}
\newcommand{\bc}{{\bf c}}
\newcommand{\be}{{\bf e}}
\newcommand{\bbf}{{\bf f}}
\newcommand{\bg}{{\bf g}}
\newcommand{\bh}{{\bf h}}
\newcommand{\bi}{{\bf i}}
\newcommand{\bj}{{\bf j}}
\newcommand{\bk}{{\bf k}}
\newcommand{\bl}{{\bf l}}
\newcommand{\bbm}{{\bf m}}
\newcommand{\bn}{{\bf n}}
\newcommand{\bp}{{\bf p}}
\newcommand{\bq}{{\bf q}}
\newcommand{\br}{{\bf r}}
\newcommand{\bu}{{\bf u}}
\newcommand{\bv}{{\bf v}}
\newcommand{\bw}{{\bf w}}
\newcommand{\bx}{{\bf x}}
\newcommand{\by}{{\bf y}}
\newcommand{\bzero}{{\bf 0}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Shorthand greek
\def\ee{\epsilon}
%%%\def\aa{\alpha}
%%%\def\bb{\beta}
\def\dd{\delta}
\def\om{\omega}
\def\ss{\sigma}
%%%\def\tt{\theta}
\def\rr{\rho}
\def\la{\lambda}
\def\Dd{\Delta}
\def\Gg{\Gamma}
\def\Om{\Omega}
\def\om{\omega}
\def\pp{\partial}
\def\veps{\varepsilon}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Boldface greek
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bfeta}{\boldsymbol{\eta}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bvarphi}{\boldsymbol{\varphi}}
\newcommand{\bzeta}{\boldsymbol{\zeta}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Math boldface-italics
\def\mathbi#1{\textbf{\em #1}}
\newcommand{\biA}{\mathbi{A}}
\newcommand{\biB}{\mathbi{B}}
\newcommand{\biC}{\mathbi{C}}
\newcommand{\biD}{\mathbi{D}}
\newcommand{\biE}{\mathbi{E}}
\newcommand{\biF}{\mathbi{F}}
\newcommand{\biG}{\mathbi{G}}
\newcommand{\biH}{\mathbi{H}}
\newcommand{\biI}{\mathbi{I}}
\newcommand{\biJ}{\mathbi{J}}
\newcommand{\biK}{\mathbi{K}}
\newcommand{\biL}{\mathbi{L}}
\newcommand{\biM}{\mathbi{M}}
\newcommand{\biN}{\mathbi{N}}
\newcommand{\biO}{\mathbi{O}}
\newcommand{\biP}{\mathbi{P}}
\newcommand{\biQ}{\mathbi{Q}}
\newcommand{\biR}{\mathbi{R}}
\newcommand{\biS}{\mathbi{S}}
\newcommand{\biT}{\mathbi{T}}
\newcommand{\biU}{\mathbi{U}}
\newcommand{\biV}{\mathbi{V}}
\newcommand{\biW}{\mathbi{W\,}}
\newcommand{\biX}{\mathbi{X}}
\newcommand{\biY}{\mathbi{Y}}
\newcommand{\biZ}{\mathbi{Z}}
%
\newcommand{\bia}{\mathbi{a}}
\newcommand{\bib}{\mathbi{b \!\!}}
\newcommand{\bic}{\mathbi{c}}
\newcommand{\bie}{\mathbi{e}}
\newcommand{\bif}{\mathbi{f\,}}
\newcommand{\bbig}{\mathbi{g}}
\newcommand{\bih}{\mathbi{h}}
\newcommand{\bii}{\mathbi{i}}
\newcommand{\bij}{\mathbi{j\,}}
\newcommand{\bik}{\mathbi{k}}
\newcommand{\bil}{\mathbi{l}}
\newcommand{\bim}{\mathbi{m}}
\newcommand{\bin}{\mathbi{n}}
\newcommand{\bip}{\mathbi{p}}
\newcommand{\biq}{\mathbi{q}}
\newcommand{\bir}{\mathbi{r}}
\newcommand{\biu}{\mathbi{u}}
\newcommand{\biv}{\mathbi{v}}
\newcommand{\biw}{\mathbi{w}}
\newcommand{\bix}{\mathbi{x}}
\newcommand{\biy}{\mathbi{y}}
\newcommand{\biz}{\mathbi{z}}
\newcommand{\bizero}{\mathbi{0}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Text boldface (Math inside theorem enviroment)
\newcommand{\tbA}{\textbf{A}}
\newcommand{\tbL}{\textbf{L}}
\newcommand{\tbU}{\textbf{U}}
\newcommand{\tbW}{\textbf{W\,}}
%
\newcommand{\tba}{\textbf{a}}
\newcommand{\tbb}{\textbf{b}}
\newcommand{\tbc}{\textbf{c}}
\newcommand{\tbd}{\textbf{d}}
\newcommand{\tbe}{\textbf{e}}
\newcommand{\tbf}{\textbf{f\,}}
\newcommand{\tbi}{\textbf{i}}
\newcommand{\tbj}{\textbf{j}}
\newcommand{\tbu}{\textbf{u}}
\newcommand{\tbv}{\textbf{v}}
\newcommand{\tbw}{\textbf{w}}
\newcommand{\tbx}{\textbf{x}}
\newcommand{\tby}{\textbf{y}}
\newcommand{\tbz}{\textbf{z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Hatted Font
\newcommand{\ha}{\hat a}
\newcommand{\hb}{\hat b}
\newcommand{\hh}{\hat h}
\newcommand{\hf}{\hat f}
\newcommand{\hg}{\hat g}
\newcommand{\hj}{\hat \jmath}
\newcommand{\hk}{\hat k}
\newcommand{\hl}{\hat l}
\newcommand{\hu}{\hat u}
\newcommand{\hs}{\hat s}
\newcommand{\hv}{\hat v}
\newcommand{\hw}{\hat w}

\newcommand{\hA}{\hat A}
\newcommand{\hD}{\hat D}
\newcommand{\hK}{\hat K}
\newcommand{\hL}{\hat L}

\newcommand{\hbiA}{\hat \biA}
\newcommand{\hbib}{\hat \bib}
\newcommand{\hbij}{\hat \bij}
\newcommand{\hbif}{\hat \bif}
\newcommand{\hIK}{\hat \IK}
\newcommand{\hcL}{\hat \cL}

\newcommand{\hgamma}{\hat \gamma}
\newcommand{\hrho}{\hat \rho}
\newcommand{\hsigma}{\hat \sigma}
\newcommand{\htau}{\hat \tau}
\newcommand{\hDelta}{\hat \Delta}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Tilded Font
\newcommand{\tell}{\tilde \ell}
\newcommand{\tJ}{\tilde J}
\newcommand{\tr}{\tilde r}
\newcommand{\tz}{\tilde z}
\newcommand{\tlambda}{\tilde \lambda}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Underlined Font
\newcommand{\un}{\underline}       % underline command.
\newcommand{\uu}{\underline u}
\newcommand{\uv}{\underline v}
\newcommand{\ux}{\underline x}
\newcommand{\uy}{\underline y}
\newcommand{\utau}{\underline \tau}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macros for Sobolev, Lebesgue etc. Spaces
\newcommand*{\Space}[3]{{#1}_{{\vphantom 1}#2}^{{\vphantom +}#3}}
\renewcommand*{\l}[2][]{\Space{L}{#1}{#2}}
\newcommand*{\h}[2][]{\Space{H}{#1}{#2}}
\newcommand*{\Lr}  [1]{\Space{L}{}{#1}(\Space{\R}{}{n})}
\newcommand*{\Lo}  [1]{\Space{L}{}{#1}(\Omega)}
\newcommand*{\Hr}  [1]{\Space{H}{}{#1}(\Space{\R}{}{n})}
\newcommand*{\Ho}  [1]{\Space{H}{}{#1}(\Omega)}
\newcommand*{\Cr}  [1]{\Space{C}{}{#1}(\Space{\R}{}{n})}
%\newcommand*{\G}[1][r]{A^{#1}\e^{\tau A}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Shorthand fractions
\newcommand{\third}{{\scriptstyle\frac{1}{3}}}
\newcommand{\twothirds}{{\scriptstyle\frac{2}{3}}}
\newcommand{\half}{{\scriptstyle 1/2}}
\newcommand{\halfs}{{\scriptstyle\frac{1}{2}}}
\newcommand{\fourth}{{\scriptstyle\frac{1}{4}}}
\newcommand{\threefourths}{{\scriptstyle\frac{3}{4}}}
\newcommand{\fifth}{{\scriptstyle\frac{1}{5}}}
\newcommand{\eighth}{{\scriptstyle\frac{1}{8}}}
\newcommand{\sixteenth}{{\scriptstyle\frac{1}{16}}}
\newcommand{\thirtysecond}{{\scriptstyle\frac{1}{32}}}
\newcommand{\fivethirds}{{\scriptstyle\frac{5}{3}}}
\newcommand{\sixfifths}{{\scriptstyle\frac{6}{5}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Other useful symbols
\newcommand{\Ahatstar}{{}^{*}\!\!\hat{A}}
\newcommand{\angstrom}{\stackrel{o}{\tiny\rm A}}
\newcommand{\PLTMG}{{\sc PLTMG}}
\newcommand{\MC}{{\sc MC}}
\newcommand{\MCX}{{\sc MCX}}
\newcommand{\MALOC}{{\sc MALOC}}
\newcommand{\SG}{{\sc SG}}
\newcommand{\MCLAB}{{\sc MCLab}}
\newcommand{\APBS}{{\sc APBS}}
\newcommand{\FETK}{{\sc FETK}}
\newcommand{\PUNC}{{\sc PUNC}}
\newcommand{\GAMER}{{\sc GAMer}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Everything else
\newcommand*{\pref}[1]{(\ref{#1})}
\newcommand*{\uh}[1]{u_h^{#1}}
\newcommand*{\Vnorm}[1]{\| #1\|_h}
\newcommand*{\paren}[1]{\left(#1\right)}
\newcommand*{\nablab}{{\bf\nabla}}
\newcommand*{\ubar}{{\bar{u}}}
\newcommand*{\uhat}{{\hat{u}}}
\newcommand*{\uns}{{\tilde{u}}}
\newcommand*{\Uns}{{\tilde{U}}}
\newcommand*{\Del}[1]{{\Delta{#1}}}
\newcommand*{\ra}{{\rightarrow}}
\newcommand*{\tone}{{\theta_1}}
\newcommand*{\ttwo}{{\theta_2}}
\newcommand{\I}{I}          
\newcommand{\II}{I\!I}          
\newcommand{\III}{I\!I\!I}          

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% END: TeX/LaTeX/PDFLaTeX <Symbols> for Holst Group Papers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


